PlotMap: Automated Layout Design for Building Game Worlds

World-building, the process of developing both the narrative and physical world of a game, plays a vital role in the game's experience. Critically-acclaimed independent and AAA video games are praised for strong world-building, with game maps that masterfully intertwine with and elevate the narrative, captivating players and leaving a lasting impression. However, designing game maps that support a desired narrative is challenging, as it requires satisfying complex constraints from various considerations. Most existing map generation methods focus on considerations about gameplay mechanics or map topography, while the need to support the story is typically neglected. As a result, extensive manual adjustment is still required to design a game world that facilitates particular stories. In this work, we approach this problem by introducing an extra layer of plot facility layout design that is independent of the underlying map generation method in a world-building pipeline. Concretely, we define (plot) facility layout tasks as the tasks of assigning concrete locations on a game map to abstract locations mentioned in a given story (plot facilities), following spatial constraints derived from the story. We present two methods for solving these tasks automatically: an evolutionary computation based approach through Covariance Matrix Adaptation Evolution Strategy (CMA-ES), and a Reinforcement Learning (RL) based approach. We develop a method of generating datasets of facility layout tasks, create a gym-like environment for experimenting with and evaluating different methods, and further analyze the two methods with comprehensive experiments, aiming to provide insights for solving facility layout tasks. We will release the code and a dataset containing 10, 000 tasks of different scales.

==> 9_figures.tex <==
\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/edge_preference_random_no_constraint.png}
    \vspace{-1mm}
    \caption{(a) Agents with no constraints; (b) Random agents.  It can be seen that the agents have a strong preference of going towards the edge of the map when there are no constraints provided in the environment. Note that the map, constraints, and initial locations are all the same for the two settings. }
    \label{fig:edge_preference}
\end{figure}

\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/task_5_different_checkpoints_Square.png}
    \vspace{-1mm}
    \caption{Motion trails at different training stages: (a) random agents; (b) after 30 iterations; (c) after 90 iterations; (d) after 133 iterations. Earlier stage models tend to have more random routes with a lot of circling back-and-forth, where later stage models tend to show clearer direction of progression.}
    \label{fig:task5_training_stage}
\end{figure}



